LLM-based Unit Test Generation via Property Retrieval

Automated unit test generation has been widely studied, with Large Language Models (LLMs) recently showing significant potential. Moreover, in the context of unit test generation, these tools prioritize high code coverage, often at the expense of practical usability, correctness, and maintainability. In response, we propose Property-Based Retrieval Augmentation, a novel mechanism that extends LLM-based Retrieval-Augmented Generation (RAG) beyond basic vector, text similarity, and graph-based methods. Our approach considers task-specific context and introduces a tailored property retrieval mechanism. Specifically, in the unit test generation task, we account for the unique structure of unit tests by dividing the test generation process into Given, When, and Then phases. When generating tests for a focal method, we not only retrieve general context for the code under test but also consider task-specific context such as pre-existing tests of other methods, which can provide valuable insights for any of the Given, When, and Then phases. This forms property relationships between focal method and other methods, thereby expanding the scope of retrieval beyond traditional RAG. We implement this approach in a tool called APT, which sequentially performs preprocessing, property retrieval, and unit test generation, using an iterative strategy where newly generated tests guide the creation of subsequent ones. We evaluated APT on 12 open-source projects with 1515 methods, and the results demonstrate that APT consistently outperforms existing tools in terms of correctness, completeness, and maintainability of the generated tests. Moreover, we introduce a novel code-context-aware retrieval mechanism for LLMs beyond general context, offering valuable insights and potential applications for other code-related tasks.

==> content/Data-Availability_Statement.tex <==
\section{Data-Availability Statement}
Our tool and experimental results are publicly available at: \url{https://anonymous.4open.science/r/PAGTest-6421/}


==> content/abstract.tex <==
% 自动化单测生成已经被广泛研究，最近基于LLM的单测生成方法展示出巨大的潜力。然而，根据最新的Survey，现有的单测生成方法tools prioritize high code coverage, often at the expense of practical usability, correct rate, and the maintainability of the generated tests. 并且这些工具集中在理解被测代码上，缺乏考虑其他。

% In response, we propose \textit{Property-Based Retrieval Augmentation for Unit Test Generation}, a novel approach that 扩展了LLM的context检索任务中的基于向量相似度的RAG方法，

%  By dividing the test generation process into the \textit{Given}, \textit{When}, and \textit{Then} phases，This method defines property relationships
% between methods, using existing test cases as references for generating new ones. It extends
% traditional vector-based retrieval by incorporating code-specific relationships such as behavioral
% similarities, structural similarities, method dependencies, and inheritance and interface implemen-
% tations among classes. Our tool, \toolname, 预处理，属性分析和检索，单测生成to enhance the \textbf{correctness}, \textbf{completeness}, and \textbf{maintainability} of the tests.
% \toolname also applies an iterative strategy, using newly generated tests to further guide subsequent test generation.


% leverages property relationships between methods to improve the quality of generated unit tests. By dividing the test generation process into the \textit{Given}, \textit{When}, and \textit{Then} phases, we ensure that the generated tests are informed by existing test cases and method relationships. Our tool, \toolname, 预处理，属性分析和检索，单测生成to enhance the \textbf{correctness}, \textbf{completeness}, and \textbf{maintainability} of the tests. \toolname also applies an iterative strategy, using newly generated tests to further guide subsequent test generation.




==> content/methodology/Infrastructure.tex <==
\subsection{Infrastructure}
% \subsection{Preprocessing}
% 这里也可以加点形式化表示？感觉没必要，不能为了表示而表示

% 因为retrieval在我们的方法中是一个很重要的部分，我们需要进行全仓库的检索任务，所有的代码的info都需要支持直接查找到相关内容，所以我们先定义了 统一代码表示模型， 使用tree-sitter对项目所有的AST进行parse，将代码转化为关系型数据表示，最终得到class、method、interface等多个元信息数据。

% class的统一表示为 文件路径 + 类名
% method的统一表示为 文件路径 + 类名 + method signature

% 1. Metainfo extraction
% 2. Scope Graph Based ref resolution
% 3. AST-Based Code Compression
%    1. Class Montage 
%     这个用于解决引用问题
%    2. Class shrink 

% 我们首先详细介绍我们的方法的基础设施，它为我们后面进行的分析和生成任务提供了根本性的支撑。无论是让LLM分析代码还是生成代码，仅仅给LLM提供目标代码片段是不够的，还需要提供适当的静态上下文。以下三个分别分别解决了"在哪里找"，"找谁？"，"找到之后提供什么信息"这三个问题。
We first introduce the infrastructure underlying our approach, which provides fundamental support for both analysis and generation tasks. When leveraging large language models (LLMs) for code analysis or generation, simply providing the target code snippet is insufficient; appropriate static context is also required. Hence, our infrastructure tackles three essential questions:  ``\textit{\textbf{Where to find?}}'',       ``\textit{\textbf{What to look for?}}'', and ``\textit{\textbf{What information to provide once found?}}''.
\begin{table}[htbp]
\centering
\caption{Schema for Java Entities}
\begin{tabularx}{\textwidth}{|l|X|}
\hline
\textbf{Entity} & \textbf{Attributes} \\ \hline
\textbf{Class} & \texttt{name}, \texttt{path}, \texttt{uri} (\texttt{path} + \texttt{name}), \texttt{methods}, \texttt{fields}, \texttt{original\_string}, \texttt{super\_class}, \texttt{super\_interfaces} \\ \hline
\textbf{Method} & \texttt{name}, \texttt{modifiers}, \texttt{params}, \texttt{return\_type}, \texttt{signature} (\texttt{modifiers} + \texttt{return\_type} + \texttt{name} + \texttt{params}), \texttt{uri} (\texttt{path} + \texttt{class} + \texttt{signature}), \texttt{original\_string} \\ \hline
\textbf{File} & \texttt{name}, \texttt{path}, \texttt{classes}, \texttt{imports} \\ \hline
\textbf{Package} & \texttt{name}, \texttt{files} \\ \hline
\end{tabularx}
\label{tab:schema}
\end{table}
\subsubsection{Metainfo Extraction}
% 无论是分析类的属性、类间的关系，还是分析单测，我们都需要将合适的代码片段提供给LLM，而原始的代码信息都在源代码中，我们无法直接进行比如获取一个方法的源代码，获取一个类的父类，获取一个单测所在的文件等这些查询操作，这些信息我们需要通过设计合理的关系型表示，从源代码中提取出关系型信息。
% \begin{wraptable}{r}{0.5\textwidth}
%     \centering
%     \caption{Schema for Java Entities}
%     \begin{tabular}{|l|p{6cm}|}
%         \hline
%         \textbf{Entity} & \textbf{Attributes} \\
%         \hline
%         \textbf{Class} & 
%         \texttt{name}, \texttt{path}, \texttt{uri} (\texttt{path} + \texttt{name}), \texttt{methods}, \texttt{fields}, \texttt{original\_string}, \texttt{super\_class}, \texttt{super\_interfaces} \\
%         \hline
%         \textbf{Method} & 
%         \texttt{name}, \texttt{modifiers}, \texttt{params}, \texttt{return\_type}, \texttt{signature} (\texttt{modifiers} + \texttt{return\_type} + \texttt{name} + \texttt{params}), \texttt{uri} (\texttt{path} + \texttt{class} + \texttt{signature}), \texttt{original\_string} \\
%         \hline
%         \textbf{File} & 
%         \texttt{name}, \texttt{path}, \texttt{classes}, \texttt{imports} \\
%         \hline
%         \textbf{Package} & 
%         \texttt{name}, \texttt{files} \\
%         \hline
%     \end{tabular}
%     \label{tab:schema}
% \end{wraptable}
For tasks such as analyzing \textit{property relationships} between methods, analyzing unit tests, or generateing unit test for focal method, it is crucial to extract relevant code snippets and pack relevant code context for the LLM. 
% The raw source code alone is insufficient for queries like retrieving a method’s source code, finding a class’s parent, or determining the file containing a unit test. To bridge this gap,
To do so, we designed relational schemas to extract structured information from the source code.
% 我们利用tree-sitter对源代码的AST进行Parse，通过遍历AST中的每个节点，维护所需要的关系型信息并存储。以Java为例，我们为它设计了如下的Scheme：
Specifically, \toolname first parses the Abstract Syntax Tree (AST) of the source code and traverse each node to maintain the necessary relational information. This extracted data is stored in a schema tailored to each language. For instance, in the case of \begin{wrapfigure}{r}{0.55\textwidth}
    \centering
    \begin{minted}[fontsize=\small, breaklines, linenos, numbersep=2pt]{json}
{
    "uri": "src/main/java/org/redisson/transaction/
    operation/set/MoveOperation.java.MoveOperation",
    "name": "MoveOperation",
    "file_path": "src/main/java/org/redisson/transaction/
    operation/set/MoveOperation.java",
    "superclasses": "SetOperation",
    "methods": [
        "[void]commit(CommandAsyncExecutor)",
        "[void]rollback(CommandAsyncExecutor)",
    ],
    "class_docstring": "\n\n@author Nikita Koksharov\n\n",
    "original_string": "", // Omitted
    "super_interfaces": [],
    "fields": [
        {
            "docstring": "",
            "modifiers": "private",
            "marker_annotations": [],
            "type": "String",
            "name": "destinationName"
        }
    ]
}
    \end{minted}
    \caption{Omitted structured metadata for the \texttt{MoveOperation} class}
    \label{fig:move_operation}
\end{wrapfigure}Java, we designed the following schema \ref{tab:schema}~\xiang{where is the schema, Table \ref{tab:schema}?}\zhangzhe{Fixed}



% 除此之外，还为TestClass、interface、abstractclass、record等上面这些类的子类设计了特定的schema。通过化源代码为关系型表示，可以帮助我们后续所有的检索任务。
We have also designed specific schemas for other code entities such as test classes, interfaces, abstract classes, and records. Converting source code into this relational form facilitates all subsequent retrieval tasks. 
% 这给后续的所有源


The provided example (Figure \ref{fig:move_operation}) shows structured metadata extracted for the Java class \texttt{MoveOperation}. This includes the class URI(Uniform Resource Identifier), its name, file path, superclass, methods, fields, super interfaces and additional documentation. By extracting and organizing code data in such a way, we enable more efficient retrieval and analysis, supporting tasks such as method relationship analysis or automatic test generation.

\subsubsection{Scope-Graph-Based Reference Resolution}
\label{sec:scope_graph}

In LLM-based code understanding and generation tasks, it is essential to provide the model with the right context. A key aspect of this is reference resolution, which involves identifying the definitions of variables within a code snippet. This helps the LLM to understand what specific identifiers represent, improving its comprehension of the code.
\xiang{present the motivation of Reference Resolution, then present methodology}\zhangzhe{fixed}


In previous code understanding tasks based on LLMs, resolving references typically relies on language-specific completion libraries, such as RepoFuse~\cite{liang2024repofuserepositorylevelcodecompletion}, which uses jedi~\cite{jedi}, an auto completion library for Python. However, these approaches are less extensible and only support Python. The Language Server Protocol (LSP) \cite{LSP} defines the protocol used between an editor or IDE with a language server, which provides language features like auto complete, go to definition, find all references, etc. However, it requires running the corresponding language parser, which is slow, resource-intensive, and involves complex communication protocols. Given these limitations, lightweight reference resolution is essential. A faster, language-agnostic approach reduces overhead and is key for handling large codebases or working with LLMs. It allows the model to find relevant definitions without the heavy cost of traditional parsers, enabling more efficient and scalable code understanding.
\xiang{highlight the importance of lightweight analysis}\zhangzhe{Fixed}

\toolname extends the capabilities of Scope Graphs \cite{neron2015theory}, which originally resolve variable definitions within the same scope. The original approach struggles with cross-class references. \toolname improves this by identifying unresolved references in any code snippet and completing the reference lookup using the constructed Metainfo Database. ~\xiang{clarify what is original scope graph, what is new.}\zhangzhe{Fixed}

% Inspired by the formal and efficient mechanisms provided by Scope Graphs \cite{neron2015theory}, which offer a theory of name resolution for handling scope and name resolution issues in complex languages.
% We have enhanced the algorithm to identify unresolved references during the name resolution process and complete the reference lookup using constructed Metainfo Database.


\paragraph{Definition}
A \textbf{Scope Graph} \( G = (N, E) \), where \( N \) is the set of nodes and \( E \) is the set of edges, provides a structured representation of lexical scopes, declarations, and references in the program.

\begin{itemize}
    \item Nodes \( N \) represent various program entities including:
    \begin{itemize}
        \item \texttt{LocalScope}: Represents a lexical scope in the program, which encapsulates a range in the source code. %and contains child scopes or declarations.
        \item \texttt{LocalDef}: Represents a local definition, such as a variable, function, or class, declared within a specific scope.
        \item \texttt{LocalImport}: Represents an import statement that brings external symbols into the current scope.
        \item \texttt{Reference}: Represents a usage of a symbol (e.g., a variable or function) within the program, which needs to be resolved to its corresponding definition or import.

    \end{itemize}
    
    \item Edges \( E \) are relationships between these entities, modeled by specific edge types:
    \begin{itemize}
        \item \texttt{ScopeToScope}: Represents the parent-child relationship between nested scopes.
        \item \texttt{DefToScope}: Links a definition (e.g., a variable or function) to the scope in which it is declared.
        \item \texttt{ImportToScope}: Connects an import statement to the target scope it references.
        \item \texttt{RefToDef} and \texttt{RefToImport}: Capture the references from a variable usage or import to its definition or imported scope.
    \end{itemize}
\end{itemize}

\paragraph{Graph Construction and Reference Resolution}

Each scope is represented as a \texttt{LocalScope} node, which encapsulates a range in the source code and contains child scopes or declarations. The following actions are executed during graph construction:

\begin{enumerate}
    \item \textbf{Scope Insertion:} As we parse the source code, each lexical scope is inserted into the graph, and its relationship to the parent scope is captured using the \texttt{ScopeToScope} edge.
    \item \textbf{Declaration Insertion:} For every symbol declaration (e.g., variable, function, or class), a corresponding \texttt{LocalDef} node is added, and a \texttt{DefToScope} edge is created to link it to the containing scope.
    \item \textbf{Reference Resolution:} When a symbol is referenced, we traverse the Scope Graph to find the corresponding \texttt{LocalDef} or \texttt{LocalImport} node by following the \texttt{RefToDef} or \texttt{RefToImport} edges. If no matching node is found within the current scope or its parent scopes, the reference is marked as unresolved.
\end{enumerate}

\paragraph{Algorithm for Unresolved Reference Detection}

To resolve references within a given code block, APT utilize a traversal algorithm on the constructed Scope Graph \( G \):

\begin{enumerate}
    \item \textbf{Reference Insertion:} For each reference \( r_i \in R_c \) (where \( R_c \) is the set of references in the code block), the reference is associated with a corresponding scope \( s_i \in S \), which represents the lexical environment where the reference is used. Each reference is inserted into the Scope Graph for resolution:
    \[
    \text{insertRef}(r_i, s_i), \quad \forall r_i \in R_c
    \]
    
    \item \textbf{Declaration Lookup:} For each reference \( r \), the algorithm first searches for a matching declaration within the current scope \( s \):
    \[
    \text{findDecl}(r, s) = \{ d \in \text{declares}(s) \mid \text{name}(d) = \text{name}(r) \}
    \]
    If no matching declaration \( d \) is found within the current scope, the search extends to other visible scopes \( s' \in S \) via the import edges in the Scope Graph, representing cross-scope references through imports or inheritance.

    \item \textbf{Unresolved Reference Detection:} If the reference \( r \) does not match any declaration in its current scope \( s \) or in any imported scopes \( s' \), it is classified as unresolved. This can be formally represented as:
    \[
    \text{resolve}(r) = \emptyset
    \]
    The algorithm identifies unresolved references by collecting all such references where the resolution fails:
    \[
    UR = \{ r \in R_c \mid \text{resolve}(r) = \emptyset \}
    \]
\end{enumerate}

% 这里可以举一个例子
% 当查找到为解析的引用时，我们构造

% 这里还差一个查找到未解析的引用之后，如何再Metainfo Database里面查找到原始定义。

% 下面这个表述有问题！
% By structuring the code analysis as a graph traversal problem, we can efficiently model complex language features such as nested scopes, imports, and variable shadowing, while maintaining generalizability across different programming languages. The formalized algorithm for unresolved reference detection ensures systematic identification and resolution of references, enhancing the extensibility and efficiency of our system.


% % 感觉这个应该在每一节单独细说啊。。。
% \subsubsection{AST-Based Code Compression}
% % 当我们通过上面的方法检索到相关的引用时？我们应该提供哪些信息？是全部都提供，还是提供哪些？考虑到LLM输入的上下文窗口长度限制，我们实现了两种机制，在不同的场景下，选择不同的信息压缩策略，能够在不损失有效信息的情况下，减少输入长度。
% % %    1. Class Montage 
% % %     这个用于解决引用问题
% % %    2. Class shrink 
% \xiang{I do not understand the relation between 4.1.2 and 4.1.3}
% When retrieving relevant references using the methods described above, it is crucial to determine what information should be provided. Should we provide all the information, or only a subset? Given the context window length limitations of LLMs, we have implemented two mechanisms that can reduce input length without losing essential information.

% \paragraph{Definition}
% The signature of a method \( m \) within \( c \) is defined as:
% \[
% \text{Sig}(m) = \text{Descriptor}(m) + \text{ReturnType}(m) + \text{Name}(m) + \text{Parameters}(m)
% \]
% This includes the method's descriptor, which encompasses access modifiers and annotations, as well as its return type, name, and input parameters.

% The signature of a class \( c \) is:
% \[
% \text{Sig}(c) = \{\text{Sig}(m_1), \dots, \text{Sig}(m_n)\} + \text{Fields}(c)
% \]
% In this context, \( \text{Fields}(c) \) represents the field declarations.
% \xiang{such representation seems very common, there is no need to describe it in details.}
% \xiang{again, why do you need to provide such information to llm}

% The definition is implicitly recursive: any inner class within \( c \) follows the same structure for its own signature, contributing to the overall \( \text{Sig}(c) \). Thus, \( \text{Sig}(c) \) captures all method signatures, fields, and any inner classes, recursively.



% % % Class Montage：将Class的信息进行抽象，只提供Class的Signature和Fields，这个适用的场景是分析单测文件时，并不知道被测的类有哪些方法和字段。以Figxxx为例，假设我们分析的测试类中引入了HashKey，但是我们并不知道HashKey有哪些方法以及方法对应的返回值，通过Class Montage机制，仅仅提供有限但是有效的信息给LLM，就可以让LLM准确地识别出被测的类和具体方法。
% \paragraph{Class Montage}
% The Class Montage mechanism abstracts class information by providing only the method signatures, fields, and inner classes, omitting method bodies and implementations. This is particularly useful when analyzing test files or external references, where the full method details might not be necessary, but an overview of the class structure is essential. 

% Formally, for a given class \( c \), the Class Montage is defined as: \( \text{ClassMontage}(c) = \text{Sig}(c) \). This approach provides the essential information—method signatures, fields, and inner classes—without overwhelming the LLM with unnecessary detail.
% For instance, in Figure \ref{fig:class_montage_of_hashkey}, we analyze the \texttt{RedisCommonBatchExecutor} class. The Class Montage mechanism abstracts this class by omitting method bodies and including only signatures, fields, and inner classes, allowing the LLM to understand the basic structure without being overwhelmed by implementation details. 
% %By using the Class Montage mechanism, we provide only the limited but essential information to the LLM, allowing it to accurately identify the tested class and its specific methods.

% \begin{figure}[h]
%     \centering
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \begin{minted}[fontsize=\small, breaklines]{java}
% public class RedisCommonBatchExecutor {
%     private final Entry entry;
%     private final AtomicInteger slots;
%     private final BatchOptions options;
%     private static int timeout(ConnectionManager connectionManager, BatchOptions options);
%     private static int retryInterval(ConnectionManager connectionManager, BatchOptions options);
%     private static int retryAttempts(ConnectionManager connectionManager, BatchOptions options);
%     @Override
%     protected void sendCommand(CompletableFuture<Void> attemptPromise, RedisConnection connection);
% }
%         \end{minted}
%         \caption{The Class Montage of \texttt{RedisCommonBatchExecutor}}
%         \label{fig:class_montage_of_hashkey}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \begin{minted}[fontsize=\small, breaklines]{java}
% public class RedisCommonBatchExecutor {
%     private final Entry entry;
%     public RedisCommonBatchExecutor() {
%         // Constructor
%     } 
    
%     private static int retryInterval(ConnectionManager connectionManager, BatchOptions options) {
%         // Implementation omitted
%     }
    
%     private static int retryAttempts(ConnectionManager connectionManager, BatchOptions options) {
%         // Implementation omitted
%     }
% }
%         \end{minted}
%         \caption{The Class Shrink of \texttt{RedisCommonBatchExecutor}}
%         \label{fig:class_shrink_of_hashkey}
%     \end{subfigure}
% \caption{\textnormal{Class Montage and Class Shrink of \texttt{RedisCommonBatchExecutor}: a comparative example illustrating two mechanisms for reducing class information. The left side shows Class Montage, which abstracts the class by including its signature and fields. The right side shows Class Shrink, which reduces the class by retaining only the methods and fields relevant to the focal method.}}
%  \label{fig:combined_class_montage_shrink}
% \end{figure}

% \paragraph{Class Shrink}
% % 将Class的信息进行缩减，站在代码结构角度（AST角度），输入一个类的某些方法名称和字段名称（包含内部类），只留下这些相关方法和字段，同时去掉其他无关的方法和字段。这个方法的适用场景是，再同一个类中，当我们通过属性检索，为focal method检索到具有属性增强关系的方法提供给LLM生成单测时，我们要提供这些方法信息给LLM，但是提供整个类的话，不但可能会超出LLM的输入窗口限制，无关的方法和信息还可能对LLM造成干扰。
% The Class Shrink mechanism reduces the class information by focusing solely on specified methods and fields, while retaining inner classes. This is particularly useful when generating unit tests. For instance, when we retrieve methods related to a focal method through \emph{property-based retrieval}, we want to provide only these related methods and fields to the LLM, rather than the entire class. Including the whole class may not only exceed the LLM’s input window but also introduce noise from unrelated methods or fields.


% % 以RedisCommonBatchExecutor为例，如figXXX所示，如果focal method是retryAttempts，当我们为它生成单测的时候，我们通过属性检索，检索到了同类中的retryInterval方法的单测可以提供参考，此时我们就可以通过Class Shrink机制，剔除无用信息，如sendCommand方法，只留下和retryAttempts有属性关系的方法retryInterval。

% Formally, Class Shrink for a given class \( c \) is defined as:
% \[
% \text{ClassShrink}(c, M, F) = \{\text{Sig}(m) \mid m \in M\} + \{\text{Fields}(c) \cap F\}
% \]
% In this context, \( M \) denotes the set of method names to retain, and \( F \) represents the set of field names to retain.

% Any inner classes within \( C \) are recursively processed in the same manner, ensuring that only the required methods and fields are retained at each level of the class hierarchy. This mechanism minimizes the input size by removing irrelevant information while preserving the essential context for the LLM.

% For example, in Figure \ref{fig:class_shrink_of_hashkey}, consider the \texttt{RedisCommonBatchExecutor} class. If the focal method is \texttt{retryAttempts}, and through \emph{property-based retrieval} we find that the \texttt{retryInterval} method is relevant, the Class Shrink mechanism will remove irrelevant methods such as the \texttt{sendCommand} and retain only the relevant methods and fields. This allows us to provide concise input to the LLM for unit test generation, while avoiding unnecessary distractions from unrelated code.

\subsubsection{AST-Based Code Compression}
When retrieving relevant references for a code snippet, it is crucial to provide only the necessary information to fit within the LLM's context window. To address this, we designed two mechanisms tailored for different scenarios: \textit{Class Montage} and \textit{Class Shrink}.\xiang{I do not understand the relation between 4.1.2 and 4.1.3}\zhangzhe{Fixed}
\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \begin{minted}[fontsize=\small, breaklines]{java}
public class RedisCommonBatchExecutor {
    private final Entry entry;
    private final AtomicInteger slots;
    private final BatchOptions options;
    private static int timeout(ConnectionManager connectionManager, BatchOptions options);
    private static int retryInterval(ConnectionManager connectionManager, BatchOptions options);
    private static int retryAttempts(ConnectionManager connectionManager, BatchOptions options);
    @Override
    protected void sendCommand(CompletableFuture<Void> attemptPromise, RedisConnection connection);
}
        \end{minted}
        \caption{The Class Montage of \texttt{RedisCommonBatchExecutor}}
        \label{fig:class_montage_of_hashkey}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \begin{minted}[fontsize=\small, breaklines]{java}
public class RedisCommonBatchExecutor {
    private final Entry entry;
    public RedisCommonBatchExecutor() {
        // Constructor
    } 
    
    private static int retryInterval(ConnectionManager connectionManager, BatchOptions options) {
        // Implementation omitted
    }
    
    private static int retryAttempts(ConnectionManager connectionManager, BatchOptions options) {
        // Implementation omitted
    }
}
        \end{minted}
        \caption{The Class Shrink of \texttt{RedisCommonBatchExecutor}}
        \label{fig:class_shrink_of_hashkey}
    \end{subfigure}
\caption{\textnormal{Class Montage and Class Shrink of \texttt{RedisCommonBatchExecutor}: a comparative example illustrating two mechanisms for reducing class information. The left side shows Class Montage, which abstracts the class by including its signature and fields. The right side shows Class Shrink, which reduces the class by retaining only the methods and fields relevant to the focal method.}}
 \label{fig:combined_class_montage_shrink}
\end{figure}
\paragraph{Class Montage}
In certain scenarios, such as analyzing test cases, APT aims to accurately map a test method to its corresponding target method. For example, given a test method, it needs to identify the method signature of the tested function, or trace through a call chain to find the final target function. In such cases, knowing just the method signatures of the class is sufficient. Additionally, when understanding code, it is often enough to know what a referenced class does without needing all the implementation details. Here, a simplified ``montage” of the class is all that is needed. \xiang{such representation seems very common, there is no need to describe it in details.}\zhangzhe{Fixed}\xiang{again, why do you need to provide such information to llm}\zhangzhe{Fixed}

\textit{Class Montage} abstracts class details by including only method signatures, fields, and inner classes, while omitting method bodies. For example, in Figure \ref{fig:class_montage_of_hashkey}, the \texttt{RedisCommonBatchExecutor} class is reduced to its signatures and fields, offering a compact representation for LLM processing.

\paragraph{Class Shrink}
When retrieving methods related to a focal method through \textit{property-based retrieval}, providing the entire class to the LLM can be inefficient due to input length limitations and the risk of overwhelming the model with irrelevant details. To address this, we designed \textit{Class Shrink} to filter out unrelated information from the class.


\textit{Class Shrink} focuses on keeping only the relevant methods and fields, discarding everything unrelated. As shown in Figure \ref{fig:class_shrink_of_hashkey}, for the \texttt{RedisCommonBatchExecutor} class, only the relevant methods like \texttt{retryAttempts} and \texttt{retryInterval} are retained, while unrelated methods like \texttt{sendCommand} are removed. This ensures the LLM focuses on relevant context without excess information.

==> content/methodology/metainfo_extraction.tex <==
\subsection{Metainfo Extraction}


\begin{wrapfigure}{r}{0.55\textwidth}
\vspace{-14pt}
    \centering
    \begin{minted}[fontsize=\footnotesize, linenos, numbersep=2pt]{json}
{
  "uri": "src/main/java/org/redisson/transaction/
  operation/set/MoveOperation.java.MoveOperation",
  "name": "MoveOperation",
  "file_path": "src/main/java/org/redisson/transaction/
  operation/set/MoveOperation.java",
  "superclasses": "SetOperation",
  "methods": [
    "[void]commit(CommandAsyncExecutor)",
    "[void]rollback(CommandAsyncExecutor)",
  ],
  "class_docstring": "@author Nikita Koksharov",
  "original_string": "", // Omitted
  "super_interfaces": [],
  "fields": [
    {
      "docstring": "",
      "modifiers": "private",
      "marker_annotations": [],
      "type": "String",
      "name": "destinationName"
    }
  ]
}
    \end{minted}
    \caption{Simplified structured metadata for the \texttt{MoveOperation} class}
    \vspace{-10pt}
    \label{fig:move_operation}
\end{wrapfigure}
% ~\xiang{where is the schema, Table \ref{tab:schema}?}\zhangzhe{Fixed}



For tasks such as analyzing \textit{property relationships} between methods, analyzing unit tests, or generateing unit test for focal method, it is crucial to extract relevant code snippets and pack relevant code context for the LLM. 
To do so, we designed relational schemas to extract structured information from the source code.

Specifically, \toolname first parses the Abstract Syntax Tree (AST) of the source code and traverse each node to maintain the necessary relational information. This extracted data is stored in a schema tailored to each language. %For instance, in the case of Java, we designed the following schema \ref{tab:schema}.
The provided example (Figure \ref{fig:move_operation}) shows structured metadata extracted for the Java class \texttt{MoveOperation}. This includes the class URI (Uniform Resource Identifier), its name, file path, superclass, methods, fields, super interfaces and additional documentation. By extracting and organizing code data in such a way, we enable more efficient retrieval and analysis, supporting tasks such as method relationship analysis or automatic test generation.
We have also designed specific schemas for other code entities such as test classes, interfaces, abstract classes, and records. Converting source code into this relational form facilitates all subsequent retrieval tasks. 



==> content/methodology/static_context_retrieval.tex <==
\subsection{Static Context Retrieval}

In the last section, \toolname address the ``\textit{\textbf{where~to~find?}}'' problem by utilizing the \textit{Metainfo Database} to save code information.
%\xiang{what does it mean?} 
However, for effective code analysis and generation, it's equally important to resolve references within the provided code snippet. This is because the LLM needs to understand the meaning of all variables, functions, or classes used, with some of which may be defined externally (e.g., global variables or imports). 
This leads to the ``\textit{\textbf{What to look for?}}'' question, which \toolname solves through \textit{Reference Resolution Based on Scope Graph}.
This process identifies externally defined entities that the LLM needs to fully comprehend the context of the code.
%\xiang{still hard to understand why we need reference resolution}\zhangzhe{fixed}
If the external information is too large for the LLM's context window, \toolname faces the ``\textit{\textbf{What information to provide?}}'' challenge, which is managed via \textit{AST-Based Code Compression}. These techniques are crucial for test case analysis, property-based retrieval, and test case generation.


\subsubsection{Reference Resolution Based on Scope Graph}
\label{sec:scope_graph}

Providing the right context is crucial in LLM-based code understanding and generation tasks. A key part of this process is reference resolution, which identifies definitions of variables, functions, or other entities within a code snippet, helping the LLM correctly interpret and comprehend the code.

Traditional reference resolution often depends on language-specific libraries, such as RepoFuse~\cite{liang2024repofuserepositorylevelcodecompletion}, which relies on tools like jedi~\cite{jedi} for Python auto-completion. These approaches, while effective, are limited in scope, supporting only specific languages. The Language Server Protocol (LSP) \cite{LSP} improves on this by providing cross-language support for features like go-to-definition and find-references, but it introduces significant overhead due to its reliance on language parsers, making it slow and resource-intensive. Given these constraints, a lightweight and language-agnostic solution is essential for supporting large-scale codebases. %and LLM integration, as it reduces processing time and resources, improving scalability and efficiency.

To solve this problem, \toolname extends the capabilities of Scope Graphs \cite{neron2015theory}, which originally focus on resolving variable definitions within a single scope. 
While traditional scope graphs struggle with cross-class references, \toolname enhances this by identifying unresolved references across classes and files, completing lookups using the Metainfo Database. 
Formally, 
% This approach enables more comprehensive and efficient reference resolution, supporting broader and more complex code analysis tasks.

\paragraph{Definition}
A \textbf{Scope Graph} \( G = (N, E) \) provides a structured representation of lexical scopes, declarations, and references in the program. 

\begin{itemize}
    \item Nodes \( N \) represent entities such as:
    \begin{itemize}
        \item \texttt{LocalScope}: A lexical scope within the code.
        \item \texttt{LocalDef}: A local definition (e.g., variable, function, or class).
        \item \texttt{LocalImport}: An import statement introducing external symbols.
        \item \texttt{Reference}: A usage of a symbol that must be resolved to its definition or import.
    \end{itemize}
    
    \item Edges \( E \) describe relationships between these entities:
    \begin{itemize}
        \item \texttt{ScopeToScope}: A parent-child relationship between scopes.
        \item \texttt{DefToScope}: Links a definition to the scope it belongs to.
        \item \texttt{ImportToScope}: Connects imports to the target scope.
        \item \texttt{RefToDef}, \texttt{RefToImport}: Capture references to definitions or imports.
    \end{itemize}
\end{itemize}

\paragraph{Graph Construction and Reference Resolution}
During graph construction, \toolname performs the following steps:

\begin{enumerate}
    \item \textbf{Scope Insertion:} Each lexical scope is inserted into the graph, with its parent-child relationships captured using \texttt{ScopeToScope} edges.
    \item \textbf{Declaration Insertion:} For every symbol declared (e.g., variable or function), a \texttt{LocalDef} node is added and linked to the appropriate scope.
    \item \textbf{Reference Resolution:} When a symbol is referenced, the graph is traversed to find its corresponding definition or import via \texttt{RefToDef} or \texttt{RefToImport} edges. Unresolved references are flagged if no match is found in the current or parent scopes.
\end{enumerate}

\paragraph{Algorithm for Reference Resolution}
To resolve references within a code block, \toolname follows this process:

\begin{enumerate}
    \item \textbf{Reference Insertion:} For each reference \( r_i \) in the code block, associate it with its lexical scope and insert it into the Scope Graph:
    \[
    \text{insertRef}(r_i, s_i)
    \]
    
    \item \textbf{Declaration Lookup:} For each reference \( r \), search for a matching declaration in the current scope \( s \). If none is found, extend the search to visible scopes via import edges:
    \[
    \text{findDecl}(r, s)
    \]

    \item \textbf{Unresolved Reference Detection:} If no matching declaration is found, classify the reference as unresolved:
    \[
    \text{resolve}(r) = \emptyset
    \]
    Collect all unresolved references:
    \[
    UR = \{ r \in R_c \mid \text{resolve}(r) = \emptyset \}
    \]

    % 
    \item \textbf{Unresolved Reference Retrieval from Metainfo Database:} For each unresolved reference \( r \in UR \), \toolname queries the \textit{Metainfo Database} to search for definitions that might exist in other classes or files:
    \[
    \text{retrieve}(r, \textit{Metainfo Database})
    \]
\end{enumerate}


\subsubsection{AST-Based Code Compression}
When retrieving relevant references for a code snippet, it is crucial to provide only the necessary information to fit within the LLM's context window. Hence, we designed two mechanisms tailored for different scenarios: \textit{Class Montage} and \textit{Class Shrink}.
% \xiang{I do not understand the relation between 4.1.2 and 4.1.3}\zhangzhe{Fixed}

\paragraph{Class Montage}
% In certain scenarios, such as analyzing test cases, \toolname aims to accurately map a test method to its corresponding target method. 
When analyzing test cases, it is necessary to map test methods to their corresponding target methods.
Specifically, given a test method, it needs to %identify the method signature of the tested function, or 
trace through the call chain to find the final target function. In such cases, knowing just the method signatures of the class is sufficient.
Additionally, when understanding code, it is often enough to know what a referenced class does without needing all the implementation details.
Here, a simplified ``montage'' of the class is sufficient for certain scenarios. %all that is needed. 
%\xiang{such representation seems very common, there is no need to describe it in details.}\zhangzhe{Fixed}\xiang{again, why do you need to provide such information to llm}\zhangzhe{Fixed}
\textit{Class Montage} abstracts implementation details by including only method signatures, fields, and inner classes, while omitting method bodies. For example, in Figure \ref{fig:class_montage_of_hashkey}, the \texttt{RedisCommonBatchExecutor} class is reduced to its signatures and fields, offering a compact representation for LLM processing.

\paragraph{Class Shrink}
When retrieving methods related to a focal method through \textit{property-based retrieval}, providing the entire class to the LLM can be inefficient due to input length limitations and the risk of overwhelming the model with irrelevant details. To address this, we designed \textit{Class Shrink} to filter out unrelated information from the class.
\textit{Class Shrink} focuses on keeping only the relevant methods and fields, discarding everything unrelated. As shown in Figure \ref{fig:class_shrink_of_hashkey}, for the \texttt{RedisCommonBatchExecutor} class \footnote{\url{https://github.com/redisson/redisson/blob/master/redisson/src/main/java/org/redisson/command/CommandBatchService.java}}, only the relevant methods like \texttt{retryAttempts} and \texttt{retryInterval} are retained, while unrelated methods like \texttt{sendCommand} are removed. This ensures the LLM focuses on relevant context without excess information.\xiang{how do you define what related method is, how to determine unrelated method.}

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \begin{minted}[fontsize=\footnotesize, breaklines]{java}
public class RedisCommonBatchExecutor {
    private final Entry entry;
    private final BatchOptions options;
    private static int timeout(ConnectionManager connectionManager, BatchOptions options);
    private static int retryInterval(ConnectionManager connectionManager, BatchOptions options);
    private static int retryAttempts(ConnectionManager connectionManager, BatchOptions options);
    @Override
    protected void sendCommand(CompletableFuture<Void> attemptPromise, RedisConnection connection);
}
        \end{minted}
        \caption{\texttt{RedisCommonBatchExecutor}'s Class Montage}
        \label{fig:class_montage_of_hashkey}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \begin{minted}[fontsize=\footnotesize, breaklines]{java}
public class RedisCommonBatchExecutor {
    private final Entry entry;
    public RedisCommonBatchExecutor() {
        // Constructor
    } 
    
    private static int retryInterval(ConnectionManager connectionManager, BatchOptions options) {
        // Implementation omitted
    }
    
    private static int retryAttempts(ConnectionManager connectionManager, BatchOptions options) {
        // Implementation omitted
    }
}
        \end{minted}
        \caption{\texttt{RedisCommonBatchExecutor}'s Class Shrink}
        \label{fig:class_shrink_of_hashkey}
    \end{subfigure}
\caption{Class Montage and Class Shrink of \texttt{RedisCommonBatchExecutor}: a comparative example illustrating two mechanisms for reducing class information. The left side shows Class Montage, which abstracts the class by including its signature and fields. The right side shows Class Shrink, which reduces the class by retaining only the methods and fields relevant to the focal method.}

 \label{fig:combined_class_montage_shrink}
\end{figure}

% \footnotetext{Source: \url{https://github.com/redisson/redisson/blob/master/redisson/src/main/java/org/redisson/command/CommandBatchService.java}}

